Demo: Multi-Modal Seizure Prediction System

This demo presents SeizNet, an innovative system for predicting epileptic seizures benefiting from a multi-modal sensor network and utilizing Deep Learning (DL) techniques. Epilepsy affects approximately 65 million people worldwide, many of whom experience drug-resistant seizures. SeizNet aims at providing highly accurate alerts, allowing individuals to take preventive measures without being disturbed by false alarms. SeizNet uses a combination of data collected through either invasive (intracranial electroencephalogram (iEEG)) or non-invasive (electroencephalogram (EEG) and electrocardiogram (ECG)) sensors, and processed by advanced DL algorithms that are optimized for real-time inference at the edge, ensuring privacy and minimizing data transmission. SeizNet achieves > 97% accuracy in seizure prediction while keeping the size and energy restrictions of an implantable device.

==> bib.tex <==
@article{iasemidis2003epileptic,
  title={Epileptic seizure prediction and control},
  author={Iasemidis, Leon D},
  journal={IEEE Transactions on Biomedical Engineering},
  volume={50},
  number={5},
  pages={549--558},
  year={2003},
  publisher={IEEE}
}


